Spatial aberrations in high-order harmonic generation

We investigate the spatial characteristics of high-order harmonic radiation generated in argon, and observe cross-like patterns in the far field. An analytical model describing harmonics from an astigmatic driving beam reveals that these patterns result from the order and generation position dependent divergence of harmonics. Even small amounts of driving field astigmatism may result in cross-like patterns, coming from the superposition of individual harmonics with spatial profiles elongated in different directions. By correcting the aberrations using a deformable mirror, we show that fine-tuning the driving wavefront is essential for optimal spatial quality of the harmonics.

==> ref.tex <==
@article{
HampusSpatioTemporal,
  title={Spatiotemporal coupling of attosecond pulses},
  author={Wikmark, Hampus and Guo, Chen and Vogelsang, Jan and Smorenburg, Peter W and Coudert-Alteirac, H{\'e}l{\`e}ne and Lahl, Jan and Peschel, Jasper and Rudawski, Piotr and Dacasa, Hugo and Carlstr{\"o}m, Stefanos and others},
  journal={Proceedings of the National Academy of Sciences},
  volume={116},
  number={11},
  pages={4779--4787},
  year={2019},
  publisher={National Acad Sciences}
}
@article{Weissenbilder2022,
 title={How to optimize high-order harmonic generation in gases},
  author={Weissenbilder, R and Carlstr{\"o}m, S and Rego, L and Guo, C and Heyl, CM and Smorenburg, P and Constant, Eric and Arnold, CL and L’huillier, A},
  journal={Nature Reviews Physics},
  volume={4},
  number={11},
  pages={713--722},
  year={2022},
  publisher={Nature Publishing Group UK London}
}

@article{2004OptimizationwithDM,
title={Optimization of high-order harmonic generation by adaptive control of a sub-10-fs pulse wave front}, volume={29},
number={2},
journal={Optics Letters},
publisher={The Optical Society},
author={Villoresi, Paolo and Bonora, Stefano and Pascolini, Michele and Poletto, Luca and Tondello, Giuseppe and Vozzi, Caterina and Nisoli, Mauro and Sansone, Giuseppe and Stagira, Salvatore and De Silvestri, Sandro}, year={2004}, month={1}, pages={207--209}, language={en} }

@article{dacasa2019single,
  title={Single-shot extreme-ultraviolet wavefront measurements of high-order harmonics},
  author={Dacasa, Hugo and Coudert-Alteirac, H{\'e}l{\`e}ne and Guo, Chen and Kueny, Emma and Campi, Filippo and Lahl, Jan and Peschel, Jasper and Wikmark, Hampus and Major, Bal{\'a}zs and Malm, Erik and others},
  journal={Optics Express},
  volume={27},
  number={3},
  pages={2656--2670},
  year={2019},
  publisher={Optica Publishing Group}
}

@article{frumker2012order,
  title={Order-dependent structure of high harmonic wavefronts},
  author={Frumker, Eug{\`e}ne and Paulus, GG and Niikura, H and Naumov, A and Villeneuve, DM and Corkum, PB},
  journal={Optics Express},
  volume={20},
  number={13},
  pages={13870--13877},
  year={2012},
  publisher={Optica Publishing Group}
}

@article{sakdinawat2010nanoscale,
  title={Nanoscale X-ray imaging},
  author={Sakdinawat, Anne and Attwood, David},
  journal={Nature photonics},
  volume={4},
  number={12},
  pages={840--848},
  year={2010},
  publisher={Nature Publishing Group UK London}
}

@article{popmintchev2012bright,
  title={Bright coherent ultrahigh harmonics in the keV x-ray regime from mid-infrared femtosecond lasers},
  author={Popmintchev, Tenio and Chen, Ming-Chang and Popmintchev, Dimitar and Arpin, Paul and Brown, Susannah and Ali{\v{s}}auskas, Skirmantas and Andriukaitis, Giedrius and Bal{\v{c}}iunas, Tadas and M{\"u}cke, Oliver D and Pugzlys, Audrius and others},
  journal={science},
  volume={336},
  number={6086},
  pages={1287--1291},
  year={2012},
  publisher={American Association for the Advancement of Science}
}

@article{Hoflund2021,
  year = {2021},
  publisher = {American Association for the Advancement of Science ({AAAS})},
  author = {M. Hoflund and Jasper Peschel and Marius Plach and Hugo Dacasa and K{\'{e}}vin Veyrinas and Eric Constant and Peter Smorenburg and Hampus Wikmark and Sylvain Maclot and Chen Guo and Cord Arnold and Anne L{\textquotesingle}Huillier and Per Eng-Johnsson},
  title = {Focusing Properties of High-Order Harmonics},
  journal = {Ultrafast Science}
}

@article{zurch2014real,
  title={Real-time and sub-wavelength ultrafast coherent diffraction imaging in the extreme ultraviolet},
  author={Z{\"u}rch, M and Rothhardt, J and H{\"a}drich, S and Demmler, S and Krebs, M and Limpert, J and T{\"u}nnermann, A and Guggenmos, Alexander and Kleineberg, Ulf and Spielmann, C},
  journal={Scientific reports},
  volume={4},
  number={1},
  pages={1--5},
  year={2014},
  publisher={Springer}
}

@article{BorregoVarillas2022,
  title={Attosecond spectroscopy for the investigation of ultrafast dynamics in atomic, molecular and solid-state physics},
  author={Borrego-Varillas, Roc{\'\i}o and Lucchini, Matteo and Nisoli, Mauro},
  journal={Reports on Progress in Physics},
  volume={85},
  number={6},
  pages={066401},
  year={2022},
  publisher={IOP Publishing}
}

@article{PhysRevA.95.063823,
  title={Tunable high-harmonic generation by chromatic focusing of few-cycle laser pulses},
  author={Holgado, Warein and Hern{\'a}ndez-Garc{\'\i}a, Carlos and Alonso, Benjam{\'\i}n and Miranda, Miguel and Silva, Francisco and Varela, O and Hern{\'a}ndez-Toro, Juan and Plaja, Luis and Crespo, Helder and Sola, IJ},
  journal={Physical Review A},
  volume={95},
  number={6},
  pages={063823},
  year={2017},
  publisher={APS}
}

@article{Milosevic:22,
  title={Macroscopic effects in high-order harmonic generation--a focal-averaging method based on the integral solution of the wave equation},
  author={Milo{\v{s}}evi{\'c}, Dejan B},
  journal={Optics Express},
  volume={30},
  number={7},
  pages={12163--12177},
  year={2022},
  publisher={Optica Publishing Group}
}

@article{PhysRevA.49.2117,
  title={Theory of high-harmonic generation by low-frequency laser fields},
  author={Lewenstein, Maciej and Balcou, Ph and Ivanov, M Yu and L’huillier, Anne and Corkum, Paul B},
  journal={Physical Review A},
  volume={49},
  number={3},
  pages={2117},
  year={1994},
  publisher={APS}
}

@article{RevModPhys.81.163,
  title={Attosecond physics},
  author={Krausz, Ferenc and Ivanov, Misha},
  journal={Reviews of modern physics},
  volume={81},
  number={1},
  pages={163},
  year={2009},
  publisher={APS}
}


@article{Dilanian2009,
  year = {2009},
  publisher = {{AIP} Publishing},
  volume = {106},
  author = {Ruben A. Dilanian and Bo Chen and Garth J. Williams and Harry M. Quiney and Keith A. Nugent and Sven Teichmann and Peter Hannaford and Lap V. Dao and Andrew G. Peele},
  title = {Diffractive imaging using a polychromatic high-harmonic generation soft-x-ray source},
  journal = {Journal of Applied Physics}
}

@article{Loetgering:22,
 title={Advances in laboratory-scale ptychography using high harmonic sources},
  author={Loetgering, Lars and Witte, Stefan and Rothhardt, Jan},
  journal={Optics Express},
  volume={30},
  number={3},
  pages={4133--4164},
  year={2022},
  publisher={Optica Publishing Group}
}

@article{Heyl_2016,
  title={Introduction to macroscopic power scaling principles for high-order harmonic generation},
  author={Heyl, CM and Arnold, CL and Couairon, Arnaud and L’Huillier, Anne},
  journal={Journal of Physics B: Atomic, Molecular and Optical Physics},
  volume={50},
  number={1},
  pages={013001},
  year={2016},
  publisher={IOP Publishing}
}

@article{Zrch2014,
  title={Real-time and sub-wavelength ultrafast coherent diffraction imaging in the extreme ultraviolet},
  author={Z{\"u}rch, M and Rothhardt, J and H{\"a}drich, S and Demmler, S and Krebs, M and Limpert, J and T{\"u}nnermann, A and Guggenmos, Alexander and Kleineberg, Ulf and Spielmann, C},
  journal={Scientific reports},
  volume={4},
  number={1},
  pages={1--5},
  year={2014},
  publisher={Springer}
}

@article{PhysRevLett.90.193901,
  title={Global optimization of high harmonic generation},
  author={Kazamias, Sophie and Douillet, D and Weihe, Frederick and Valentin, C and Rousse, Antoine and Sebban, St{\'e}phane and Grillon, G and Aug{\'e}, F and Hulin, D and Balcou, Ph},
  journal={Physical Review Letters},
  volume={90},
  number={19},
  pages={193901},
  year={2003},
  publisher={APS}
}

@article{PhysRevLett.81.297,
  title = {Temporal Coherence of Ultrashort High-Order Harmonic Pulses},
  author = {Bellini, M. and Lyng\aa{}, C. and Tozzi, A. and Gaarde, M. B. and H\"ansch, T. W. and L'Huillier, A. and Wahlstr\"om, C.-G.},
  journal = {Phys. Rev. Lett.},
  volume = {81},
  year = {1998},
  publisher = {American Physical Society},
}


@article{PhysRevA.51.1495,
  title = {Rings in above-threshold ionization: A quasiclassical analysis},
  author = {Lewenstein, M. and Kulander, K. C. and Schafer, K. J. and Bucksbaum, P. H.},
  journal = {Phys. Rev. A},
  volume = {51},
  year = {1995},
  publisher = {American Physical Society},
}



@article{PhysRevLett.74.3776,
  title = {Coherence Control of High-Order Harmonics},
  author = {Sali\`eres, P. and L'Huillier, Anne and Lewenstein, Maciej and AA},
  journal = {Phys. Rev. Lett.},
  year = {1995},
  publisher = {American Physical Society},
}


@article{Carlstrm2016,
  title={Spatially and spectrally resolved quantum path interference with chirped driving pulses},
  author={Carlstr{\"o}m, Stefanos and Precl{\'\i}kov{\'a}, Jana and Lorek, Eleonora and Larsen, Esben Witting and Heyl, Christoph M and Pale{\v{c}}ek, David and Zigmantas, Donatas and Schafer, Kenneth J and Gaarde, Mette B and Mauritsson, Johan},
  journal={New Journal of Physics},
  volume={18},
  number={12},
  pages={123032},
  year={2016},
  publisher={IOP Publishing}
}


@article{Guo2018,
  title={Phase control of attosecond pulses in a train},
  author={Guo, Chen and Harth, Anne and Carlstr{\"o}m, Stefanos and Cheng, Yu-Chen and Mikaelsson, Sara and Marsell, Erik and Heyl, Christoph and Miranda, Miguel and Gisselbrecht, Mathieu and Gaarde, Mette B and others},
  journal={Journal of Physics B: Atomic, Molecular and Optical Physics},
  volume={51},
  number={3},
  pages={034006},
  year={2018},
  publisher={IOP Publishing}
}

@article{PhysRevLett.71.1994,
  title={Plasma perspective on strong field multiphoton ionization},
  author={Corkum, Paul B},
  journal={Physical review letters},
  volume={71},
  number={13},
  pages={1994},
  year={1993},
  publisher={APS}
}

@article{PhysRevLett.70.1599,
  title={Above threshold ionization beyond the high harmonic cutoff},
  author={Schafer, KJ and Yang, Baorui and DiMauro, LF and Kulander, KC},
  journal={Physical review letters},
  volume={70},
  number={11},
  pages={1599},
  year={1993},
  publisher={APS}
}

@article{PhysRevLett.68.3535,
  title={High-order harmonic generation from atoms and ions in the high intensity regime},
  author={Krause, Jeffrey L and Schafer, Kenneth J and Kulander, Kenneth C},
  journal={Physical Review Letters},
  volume={68},
  number={24},
  pages={3535},
  year={1992},
  publisher={APS}
}

@article{Ferray1988,
  year = {1988},
  publisher = {{IOP} Publishing},
  volume = {21},
  author = {M Ferray and A L{\textquotesingle}Huillier and X F Li and L A Lompre and G Mainfray and C Manus},
  title = {Multiple-harmonic conversion of 1064 nm radiation in rare gases},
  journal = {Journal of Physics B: Atomic,  Molecular and Optical Physics}
}

@article{Gaarde2008,
  year = {2008},
  publisher = {{IOP} Publishing},
  volume = {41},
  number = {13},
  author = {Mette B Gaarde and Jennifer L Tate and Kenneth J Schafer and Nobody else},
  title = {Macroscopic aspects of attosecond pulse generation},
  journal = {Journal of Physics B: Atomic,  Molecular and Optical Physics}
}

@article{McPherson:87,
author = {A. McPherson and G. Gibson and H. Jara and U. Johann and T. S. Luk and I. A. McIntyre and K. Boyer and C. K. Rhodes},
journal = {J. Opt. Soc. Am. B},
number = {4},
publisher = {Optica Publishing Group},
title = {Studies of multiphoton production of vacuum-ultraviolet radiation in the rare gases},
volume = {4},
year = {1987},
abstract = {Measurements of the vacuum-ultraviolet (\&lt;80-nm) radiation produced by intense ultraviolet (248-nm) irradiation (1015--1016 W/cm2) of rare gases have revealed the copious presence of both harmonic radiation and fluorescence from excited levels. The highest harmonic observed was the seventeenth (14.6 nm) in Ne, the shortest wavelength ever produced by that means. Strong fluorescence was seen from ions of Ar, Kr, and Xe, with the shortest wavelengths observed being below 12 nm. Furthermore, radiation from inner-shell excited configurations in Xe, specifically the 4d95s5p 4d105s manifold of Xe7$+$ at ~17.7 nm, was detected. These experimental findings, in alliance with other studies concerning multielectron processes, give evidence for a role of electron correlations in a direct nonlinear process of inner-shell excitation.},
}

@article{Kochkina:13,
 title={Modeling of the general astigmatic Gaussian beam and its propagation through 3D optical systems},
  author={Kochkina, Evgenia and Wanner, Gudrun and Schmelzer, Dennis and Tr{\"o}bs, Michael and Heinzel, Gerhard},
  journal={Applied optics},
  volume={52},
  number={24},
  pages={6030--6040},
  year={2013},
  publisher={Optical Society of America}
}
@article{PhysRevLett.117.163202,
  title={Nonperturbative twist in the generation of extreme-ultraviolet vortex beams},
  author={Rego, Laura and San Rom{\'a}n, Julio and Pic{\'o}n, Antonio and Plaja, Luis and Hern{\'a}ndez-Garc{\'\i}a, Carlos},
  journal={Physical review letters},
  volume={117},
  number={16},
  pages={163202},
  year={2016},
  publisher={APS}
}


@article{HernndezGarca2015,
  title={Quantum-path signatures in attosecond helical beams driven by optical vortices},
  author={Hern{\'a}ndez-Garc{\'\i}a, Carlos and San Rom{\'a}n, J and Plaja, L and Pic{\'o}n, Antonio},
  journal={New Journal of Physics},
  volume={17},
  number={9},
  pages={093029},
  year={2015},
  publisher={IOP Publishing}
}


@article{doi:10.1126/science.108836,
author = {P. Salières  and B. Carré  and L. Le Déroff  and F. Grasbon  and G. G. Paulus  and H. Walther  and R. Kopold  and W. Becker  and D. B. Milošević  and A. Sanpera  and M. Lewenstein },
title = {Feynman's Path-Integral Approach for Intense-Laser-Atom Interactions},
journal = {Science},
volume = {292},
year = {2001},
}

@article{Ensemble2022,
  year = {2022},
  month = jun,
  publisher = {{IOP} Publishing},
  volume = {4},
  number = {3},
  pages = {034006},
  author = {F. Vismarra and R. Borrego-Varillas and Y. Wu and D. Mocci and M. Nisoli and M. Lucchini},
  title = {Ensemble effects on the reconstruction of attosecond pulses and photoemission time delays},
  journal = {Journal of Physics: Photonics}
}

@article{PhysRevA.93.061402,
  title = {Two-photon double ionization of neon using an intense attosecond pulse train},
  author = {Manschwetus, B. and Rading, L. and Campi, F. and Maclot, S. and Coudert-Alteirac, H. and Lahl, J. and Wikmark, H. and Rudawski, P. and Heyl, C. M. and Farkas, B. and Mohamed, T. and L'Huillier, A. and Johnsson, P.},
  journal = {Phys. Rev. A},
  volume = {93},
  issue = {6},
  pages = {061402},
  numpages = {5},
  year = {2016},
  month = {6},
  publisher = {American Physical Society}
}

@article{Veyrinas2023,
  title={Chromatic aberrations correction of attosecond high-order harmonic beams by flat-top spatial shaping of the fundamental beam},
  author={Veyrinas, K and Plach, M and Peschel, J and Hoflund, M and Catoire, F and Valentin, C and Smorenburg, P and Dacasa, H and Maclot, S and Guo, C and others},
  journal={New Journal of Physics},
  volume={25},
  number={2},
  pages={023017},
  year={2023},
  publisher={IOP Publishing}
}

@article{ValentinJOSAB2008,
  title={High-order harmonic wave fronts generated with controlled astigmatic infrared laser},
  author={Valentin, Constance and Gautier, Julien and Goddet, Jean-Philippe and Hauri, Christoph and Marchenko, Tatiana and Papalazarou, Evaggelos and Rey, Gilles and Sebban, St{\'e}phane and Scrick, Oph{\'e}lie and Zeitoun, Philippe and others},
  journal={JOSA B},
  volume={25},
  number={7},
  pages={B161--B166},
  year={2008},
  publisher={Optica Publishing Group}
}

@article{QuintardSciAdv2019,
author = {L. Quintard  and V. Strelkov  and J. Vabek  and O. Hort  and A. Dubrouil  and D. Descamps  and F. Burgy  and C. Péjot  and E. Mével  and F. Catoire  and E. Constant },
title = {Optics-less focusing of XUV high-order harmonics},
journal = {Science Advances},
volume = {5},
number = {4},
pages = {eaau7175},
year = {2019},
doi = {10.1126/sciadv.aau7175},
URL = {https://www.science.org/doi/abs/10.1126/sciadv.aau7175},
eprint = {https://www.science.org/doi/pdf/10.1126/sciadv.aau7175},
}

@article{Wodzinski:20,
author = {Thomas Wodzinski and Swen K\"{u}nzel and Jayanath C. P. Koliyadu and Mukhtar Hussain and Barbara Keitel and Gareth O. Williams and Philippe Zeitoun and Elke Pl\"{o}njes and Marta Fajardo},
journal = {Appl. Opt.},
keywords = {Deformable mirrors; Gas lasers; Infrared lasers; Plasma diagnostics; Soft x rays; Wavefronts},
number = {5},
pages = {1363--1370},
publisher = {Optica Publishing Group},
title = {High-harmonic generation wave front dependence on a driving infrared wave front},
volume = {59},
month = {2},
year = {2020},
url = {https://opg.optica.org/ao/abstract.cfm?URI=ao-59-5-1363},
doi = {10.1364/AO.59.001363},
}

@article{Kretschmar:20,
author = {Martin Kretschmar and Johannes Tuemmler and Bernd Sch\"{u}tte and Andreas Hoffmann and Bj\"{o}rn Senfftleben and Mark Mero and Mario Sauppe and Daniela Rupp and Marc J. J. Vrakking and Ingo Will and Tamas Nagy},
journal = {Opt. Express},
keywords = {Extreme ultraviolet; Hollow core fibers; Nd:YAG lasers; Optical parametric chirped pulse amplification; Regenerative amplification; Yb:YAG lasers},
number = {23},
pages = {34574--34585},
publisher = {Optica Publishing Group},
title = {Thin-disk laser-pumped OPCPA system delivering 4.4 TW few-cycle pulses},
volume = {28},
month = {11},
year = {2020},
url = {https://opg.optica.org/oe/abstract.cfm?URI=oe-28-23-34574},
doi = {10.1364/OE.404077},
}

@article{Miao15,
author = {Jianwei Miao  and Tetsuya Ishikawa  and Ian K. Robinson  and Margaret M. Murnane },
title = {Beyond crystallography: Diffractive imaging using coherent x-ray light sources},
journal = {Science},
volume = {348},
number = {6234},
pages = {530-535},
year = {2015},
doi = {10.1126/science.aaa1394},
URL = {https://www.science.org/doi/abs/10.1126/science.aaa1394},
eprint = {https://www.science.org/doi/pdf/10.1126/science.aaa1394},
}

@article{Makos2020,
  title={A 10-gigawatt attosecond source for non-linear XUV optics and XUV-pump-XUV-probe studies},
  author={Makos, Ioannis and Orfanos, I and Nayak, Arjun and Peschel, Jasper and Major, Bal{\'a}zs and Liontos, Ioannis and Skantzakis, Emmanuel and Papadakis, N and Kalpouzos, Constantinos and Dumergue, Mathieu and others},
  journal={Scientific reports},
  volume={10},
  number={1},
  pages={3759},
  year={2020},
  publisher={Nature Publishing Group UK London}
}

@article{kretschmar2023compact,
  title={Compact realization of all-attosecond pump-probe spectroscopy},
  author={Kretschmar, Martin and Svirplys, Evaldas and Volkov, Mikhail and Witting, Tobias and Nagy, Tam{\'a}s and Vrakking, Marc JJ and Sch{\"u}tte, Bernd},
  journal={arXiv preprint arXiv:2306.16212},
  year={2023}
}

@article{Gardner2017,
  doi = {10.1038/nphoton.2017.33},
  url = {https://doi.org/10.1038/nphoton.2017.33},
  year = {2017},
  month = mar,
  publisher = {Springer Science and Business Media {LLC}},
  volume = {11},
  number = {4},
  pages = {259--263},
  author = {Dennis F. Gardner and Michael Tanksalvala and Elisabeth R. Shanblatt and Xiaoshi Zhang and Benjamin R. Galloway and Christina L. Porter and Robert Karl Jr and Charles Bevis and Daniel E. Adams and Henry C. Kapteyn and Margaret M. Murnane and Giulia F. Mancini},
  title = {Subwavelength coherent imaging of periodic samples using a 13.5{\hspace{0.25em}}nm tabletop high-harmonic light source},
  journal = {Nature Photonics}
}
